DYPLOC: Dynamic Planning of Content Using Mixed Language Models for Text Generation

We study the task of long-form opinion text generation, which faces at least two distinct challenges. First, existing neural generation models fall short of coherence, thus requiring efficient content planning. Second, diverse types of information are needed to guide the generator to cover both subjective and objective content. To this end, we propose DYPLOC, a generation framework that conducts dynamic planning of content while generating the output based on a novel design of mixed language models. To enrich the generation with diverse content, we further propose to use large pre-trained models to predict relevant concepts and to generate claims. We experiment with two challenging tasks on newly collected datasets: (1) argument generation with Reddit ChangeMyView, and (2) writing articles using New York Times' Opinion section. Automatic evaluation shows that our model significantly outperforms competitive comparisons. Human judges further confirm that our generations are more coherent with richer content.

==> bakup.tex <==
\begin{table*}[t]
\centering
\fontsize{10}{12}\selectfont
\small
 \setlength{\tabcolsep}{1.5mm}
\centering
    
    \begin{tabular}{l llll l llll}
    \toprule
        & \multicolumn{4}{c}{Argument Generation (CMV)} & \phantom{} & \multicolumn{4}{c}{Opinion Article Generation (NYT)} \\
        
        & \bf{BLEU-2} & \bf{ROUGE-2} & \bf{METEOR} & \bf{Len.} & \phantom{} & \bf{BLEU-2} & \bf{ROUGE-2} & \bf{METEOR} & \bf{Len.} \\
        \midrule
        \textsc{Retrieval} & 6.29 & 3.68 & 10.00 & 78 & \phantom{} & 9.68 & 7.96 & 9.98 & 99 \\ 
        \textsc{SentPlanner} & 7.78 & 3.23 & 7.69 & 114 & \phantom{} & 7.45 & 5.06  & 6.62  & 106 \\ 
        \textsc{Seq2seq} & 16.71 & 9.53 & 13.34 & 100 & \phantom{} & 21.44 & 14.92 & 14.93 & 119 \\
        \textsc{Seq2seqFull} & 29.11 & 17.71 & 20.27 & 145 & \phantom{} & 31.06 & 29.74 & 23.10 & 121 \\ 
        \midrule
        \textsc{DYPLOC} (ours)  & {\bf 32.60} & {\bf 25.69} & {\bf 22.61} & 101 & \phantom{} & {\bf 40.63} & {\bf 36.93} & 25.76 & 122  \\
        \quad w/o All Concepts & 7.80 & 3.68 & 7.21 & 107 & \phantom{} & 11.32 & 6.01 & 8.33 & 132 \\
        \quad w/o Augmented Concepts & 22.39 & 15.90 & 16.91 & 99 & \phantom{} & 26.94 & 21.56 & 18.39 & 117 \\
        \quad w/o Claims & 31.62 & 25.03 & 22.09 & 100 & \phantom{} & 39.44 & 35.43 & 25.25 & 122 \\ 
        \quad w/o Entities & 32.11 & 25.36 & 22.42 & 101 & \phantom{} & 39.66 & 35.82 & 25.11 & 122 \\ 
        \midrule
        \quad with Random Selection & 12.96 & 8.25 & 10.05 & 103 & \phantom{} & 5.32 & 5.29 & 6.00 & 72 \\ 
        \quad with Greedy Selection & 32.33 & 25.60 & 22.53 & 100 & \phantom{} & 40.61 & 36.88 & {\bf 25.77} & 122 \\
        \bottomrule
    \end{tabular}
    % \vspace{-2mm}
    \caption{
    % \lu{move to prev page}
    Automatic evaluation results on both tasks. We report BLEU-2, ROUGE-2, METEOR, and output length. Best scores are in bold. Our \textsc{DYPLOC} model statistically significantly outperforms all baselines and comparisons (randomization approximation test~\cite{noreen1989computer}, $p < 0.0005$).\xinyu{last two rows are newly added, in each step, the content item is hard-selected (randomly or the one with highest score) instead of weighted-sum.}
  }
    \label{tab:main-results}
%   \vspace{-2mm}
\end{table*}

\begin{table}[t]
    \centering
    \fontsize{10}{11}\selectfont
    \small
 \setlength{\tabcolsep}{1.4mm}
    \begin{tabular}{l D{,}{.}{2.2}D{,}{.}{2.2} D{,}{.}{2.2}D{,}{.}{2.2}}
        \toprule
        & \multicolumn{2}{c}{CMV} & \multicolumn{2}{c}{NYT} \\
         &  {\bf BLEU-2} & {\bf MTR} & {\bf BLEU-2} & {\bf MTR} \\
         \midrule
        \textsc{Retrieval} & 8,30 & 9,64 & 8.85 & 9.21 \\
        \textsc{SentPlanner} & 7.84 & 7.76 & 7.75 & 6.80 \\
        \textsc{Seq2seqFull} & 18.06 & 15.96 & 16.20 & 15.25 \\
        \textsc{DYPLOC} & {\bf 22.84} & {\bf 17.13} & {\bf 24.54} & {\bf 17.41} \\
        \bottomrule
    \end{tabular}
    % \vspace{-2mm}
    \caption{BLEU-2 and METEOR (MTR) results on systems with predicted concepts as input. Same trends are observed on ROUGE, which are in the Supplementary.}
    \label{tab:system}
\end{table}

